Brane Tilings, M2-branes and Orbifolds

Brane Tilings represent one of the largest classes of superconformal theories with known gravity duals in 3+1 and also 2+1 dimensions. They provide a useful link between a large class of quiver gauge theories and their moduli spaces, which are the toric Calabi-Yau (CY) singularities. This thesis includes a discussion of an algorithm that can be used to generate all brane tilings with any given number of superpotential terms. All tilings with at most 8 superpotential terms have been generated using an implementation of this method. Orbifolds are a subject of central importance in string theory. It is widely known that there may be two or more orbifolds of a space by a finite group. Abelian Calabi-Yau orbifolds of the form $\BC^3 / \Gamma$ can be counted according to the size of the group $|\Gamma|$. Three methods of counting these orbifolds will be given. A brane tiling together with a set of Chern Simons levels is sufficient to define a quiver Chern-Simons theory which describes the worldvolume theory of the M2-brane probe. A forward algorithm exists which allows us to easily compute the toric data associated to the moduli space of the quiver Chern-Simons theory from knowledge of the tiling and Chern-Simons levels. This forward algorithm will be discussed and illustrated with a few examples. It is possible that two different Chern-Simons theories have the same moduli-space. This effect, sometimes known as `toric duality' will be described further. We will explore how two Chern--Simons theories (corresponding to brane tilings) can be related to each other by the Higgs mechanism and how brane tilings (with CS levels) that correspond to 14 fano 3-folds have been constructed. The idea of `child' and `parent' brane tilings will be introduced and we will discuss how it has been possible to count `children' using the symmetry of the `parent' tiling.

==> bibitems.tex <==
\bibitem{Maldacena:1997re}
  J.~M.~Maldacena,
``The Large N limit of superconformal field theories and supergravity,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 2} (1998) 231
  [Int.\ J.\ Theor.\ Phys.\  {\bf 38} (1999) 1113]
  [arXiv:hep-th/9711200].


\bibitem{Gimon:1996rq}
  E.~G.~Gimon and J.~Polchinski,
``Consistency conditions for orientifolds and d manifolds,''
  Phys.\ Rev.\  D {\bf 54} (1996) 1667
  [arXiv:hep-th/9601038].

\bibitem{Polchinski:1995mt}
  J.~Polchinski,
``Dirichlet Branes and Ramond-Ramond charges,''
  Phys.\ Rev.\ Lett.\  {\bf 75} (1995) 4724
  [arXiv:hep-th/9510017].

\bibitem{Benna:2009xd}
  M.~K.~Benna, I.~R.~Klebanov and T.~Klose,
  ``Charges of Monopole Operators in Chern-Simons Yang-Mills Theory,''
  JHEP {\bf 1001} (2010) 110
  [arXiv:0906.3008 [hep-th]].

\bibitem{Jafferis:2009th}
  D.~L.~Jafferis,
``Quantum corrections to N=2 Chern-Simons theories with flavor and their
AdS(4) duals,''
  arXiv:0911.4324 [hep-th].

\bibitem{Gaiotto:2007qi}
  D.~Gaiotto and X.~Yin,
``Notes on superconformal Chern-Simons-Matter theories,''
  JHEP {\bf 0708} (2007) 056
  [arXiv:0704.3740 [hep-th]].

\bibitem{Kapustin:1994mt}
  A.~N.~Kapustin and P.~I.~Pronin,
``Nonrenormalization theorem for gauge coupling in (2+1)-dimensions,''
  Mod.\ Phys.\ Lett.\  A {\bf 9} (1994) 1925
  [arXiv:hep-th/9401053].

\bibitem{Franco:2005sm}
  S.~Franco, A.~Hanany, D.~Martelli, J.~Sparks, D.~Vegh and B.~Wecht,
 ``Gauge theories from toric geometry and brane tilings,''
  JHEP {\bf 0601}, 128 (2006)
  [arXiv:hep-th/0505211].

\bibitem{gaugefromtoric}
  S.~Franco, A.~Hanany, D.~Martelli, J.~Sparks, D.~Vegh and B.~Wecht,
  ``Gauge theories from toric geometry and brane tilings,''
  JHEP {\bf 0601} (2006) 128
  [arXiv:hep-th/0505211].

\bibitem{Hanany:2005hq}
  A.~Hanany, P.~Kazakopoulos and B.~Wecht,
  ``A new infinite class of quiver gauge theories,''
  JHEP {\bf 0508} (2005) 054
  [arXiv:hep-th/0503177].

\bibitem{pprogram}
  B.~Feng, A.~Hanany and Y.~H.~He,
  ``Counting Gauge Invariants: the Plethystic Program,''
  JHEP {\bf 0703} (2007) 090
  [arXiv:hep-th/0701063].

\bibitem{chiralops}
  A.~Butti, D.~Forcella, A.~Hanany, D.~Vegh and A.~Zaffaroni,
  ``Counting Chiral Operators in Quiver Gauge Theories,''
  JHEP {\bf 0711} (2007) 092
  [arXiv:0705.2771 [hep-th]].

\bibitem{orientifolds}
  S.~Franco, A.~Hanany, D.~Krefl, J.~Park, A.~M.~Uranga and D.~Vegh,
  ``Dimers and Orientifolds,''
  JHEP {\bf 0709} (2007) 075
  [arXiv:0707.0298 [hep-th]].

\bibitem{master3}
  D.~Forcella, A.~Hanany and A.~Zaffaroni,
  ``Master Space, Hilbert Series and Seiberg Duality,''
  arXiv:0810.4519 [hep-th].

\bibitem{ZPQ}
  T.~Oota and Y.~Yasui,
  ``New example of infinite family of quiver gauge theories,''
  Nucl.\ Phys.\  B {\bf 762} (2007) 377
  [arXiv:hep-th/0610092].

\bibitem{ypq}
  A.~Butti, D.~Forcella and A.~Zaffaroni,
  ``The dual superconformal theory for L(p,q,r) manifolds,''
  JHEP {\bf 0509} (2005) 018
  [arXiv:hep-th/0505220].

\bibitem{amaxiszmin}
  A.~Butti and A.~Zaffaroni,
  ``R-charges from toric diagrams and the equivalence of a-maximization and
  Z-minimization,''
  JHEP {\bf 0511} (2005) 019
  [arXiv:hep-th/0506232].

\bibitem{0608050}
  S.~Benvenuti, B.~Feng, A.~Hanany and Y.~H.~He,
  ``Counting BPS operators in gauge theories: Quivers, syzygies and
  plethystics,''
  JHEP {\bf 0711} (2007) 050
  [arXiv:hep-th/0608050].

\bibitem{Plog}
  D.~Forcella, A.~Hanany and A.~Zaffaroni,
  ``Baryonic generating functions,''
  JHEP {\bf 0712} (2007) 022
  [arXiv:hep-th/0701236].

\bibitem{EasyMax1}
  S.~Benvenuti, L.~A.~Pando Zayas and Y.~Tachikawa,
  ``Triangle anomalies from Einstein manifolds,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 10} (2006) 395
  [arXiv:hep-th/0601054].

\bibitem{EasyMax2}
  S.~Lee and S.~J.~Rey,
  ``Comments on anomalies and charges of toric-quiver duals,''
  JHEP {\bf 0603} (2006) 068
  [arXiv:hep-th/0601223].

\bibitem{Zonotope}
  A.~Kato,
  ``Zonotopes and four-dimensional superconformal field theories,''
  JHEP {\bf 0706} (2007) 037
  [arXiv:hep-th/0610266].

\bibitem{AmaxZmin}
  A.~Butti and A.~Zaffaroni,
  ``From toric geometry to quiver gauge theory: The equivalence of
  a-maximization and Z-minimization,''
  Fortsch.\ Phys.\  {\bf 54} (2006) 309
  [arXiv:hep-th/0512240].

\bibitem{Fulton}
  W.~Fulton,
  ``Introduction to Toric Varieties,''
  Princeton University Press, 1993.

\bibitem{Gulotta}
  D.~R.~Gulotta,
  ``Properly ordered dimers, $R$-charges, and an efficient inverse algorithm,''
  JHEP {\bf 0810} (2008) 014
  [arXiv:0807.3012 [hep-th]].

\bibitem{Masterspace}
  D.~Forcella, A.~Hanany, Y.~H.~He and A.~Zaffaroni,
  ``The Master Space of N=1 Gauge Theories,''
  JHEP {\bf 0808} (2008) 012
  [arXiv:0801.1585 [hep-th]].

\bibitem{MMasterspace}
  D.~Forcella, A.~Hanany, Y.~H.~He and A.~Zaffaroni,
  ``Mastering the Master Space,''
  Lett.\ Math.\ Phys.\  {\bf 85} (2008) 163
  [arXiv:0801.3477 [hep-th]].

\bibitem{Hanany05}
  S.~Franco, A.~Hanany, K.~D.~Kennaway, D.~Vegh and B.~Wecht,
 ``Brane Dimers and Quiver Gauge Theories,''
  JHEP {\bf 0601}, 096 (2006)
  [arXiv:hep-th/0504110].

\bibitem{Hanany:2005ss}
  A.~Hanany and D.~Vegh,
 ``Quivers, tilings, branes and rhombi,''
  JHEP {\bf 0710}, 029 (2007)
  [arXiv:hep-th/0511063].

\bibitem{FengToric}
  B.~Feng, A.~Hanany and Y.~H.~He,
  ``D-brane gauge theories from toric singularities and toric duality,''
  Nucl.\ Phys.\  B {\bf 595} (2001) 165
  [arXiv:hep-th/0003085].

\bibitem{FrancoToric}
  S.~Franco and A.~Hanany,
  ``Toric duality, Seiberg duality and Picard-Lefschetz transformations,''
  Fortsch.\ Phys.\  {\bf 51} (2003) 738
  [arXiv:hep-th/0212299].

\bibitem{AMax}
  K.~Intriligator and B.~Wecht,
  ``The exact superconformal R-symmetry maximizes a,''
  Nucl.\ Phys.\  B {\bf 667} (2003) 183
  [arXiv:hep-th/0304128].

\bibitem{Amax2}
  D.~Kutasov,
 ``New results on the 'a-theorem' in four dimensional supersymmetric field
 theory,''
  arXiv:hep-th/0312098.

\bibitem{Tachion}
  P.~S.~Aspinwall and I.~V.~Melnikov,
``D-branes on vanishing del Pezzo surfaces,''
  JHEP {\bf 0412} (2004) 042
  [arXiv:hep-th/0405134].

\bibitem{FractionalDuals}
  B.~Feng, A.~Hanany, Y.~H.~He and A.~Iqbal,
  ``Quiver theories, soliton spectra and Picard-Lefschetz transformations,''
  JHEP {\bf 0302} (2003) 056
  [arXiv:hep-th/0206152].

\bibitem{Mutations}
  C.~P.~Herzog,
  ``Seiberg duality is an exceptional mutation,''
  JHEP {\bf 0408} (2004) 064
  [arXiv:hep-th/0405118].

\bibitem{Franco:2008um}
  S.~Franco, A.~Hanany, J.~Park, D.~Rodriguez-Gomez,
  ``Towards M2-brane Theories for Generic Toric Singularities,''
  JHEP {\bf 0812 } (2008)  110.
  [arXiv:0809.3237 [hep-th]].

\bibitem{YangsTeam}
  J.~Hewlett and Y.~H.~He,
``Probing the Space of Toric Quiver Theories,''
  arXiv:0909.2879 [hep-th].

\bibitem{Davey:2009sr}
  J.~Davey, A.~Hanany, N.~Mekareeya and G.~Torri,
``Phases of M2-brane Theories,''
  JHEP {\bf 0906} (2009) 025
  [arXiv:0903.3234 [hep-th]].

\bibitem{Feng:2005gw}
  B.~Feng, Y.~-H.~He, K.~D.~Kennaway {\it et al.},
  ``Dimer models from mirror symmetry and quivering amoebae,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 12 } (2008)  3.
  [hep-th/0511287].

\bibitem{Stienstra:2007dy}
  J.~Stienstra,
 ``Hypergeometric Systems in two Variables, Quivers, Dimers and Dessins
 d'Enfants,''
  arXiv:0711.0464 [math.AG].

\bibitem{ToricD}
  B.~Feng, S.~Franco, A.~Hanany and Y.~H.~He,
``Symmetries of toric duality,''
  JHEP {\bf 0212} (2002) 076
  [arXiv:hep-th/0205144].

\bibitem{Satake}
 I.~Satake,
 ``On a Generalization of the notion of manifold,''
 Proc. Natl. Acad. Sci. USA. 1956 June; 42(6): 359�363. 

\bibitem{Thurston}
 W.~P.~Thurston,
 ``The Geometry and Topologt of Three-Manifolds,''
 Princeton, 1978.

\bibitem{preDixon}
  L.~J.~Dixon, J.~A.~Harvey, C.~Vafa and E.~Witten,
 ``Strings On Orbifolds,''
  Nucl.\ Phys.\  B {\bf 261} (1985) 678.

\bibitem{postDixon}
  L.~J.~Dixon, J.~A.~Harvey, C.~Vafa and E.~Witten,
 ``Strings On Orbifolds. 2,''
  Nucl.\ Phys.\  B {\bf 274} (1986) 285.

\bibitem{Dixon:1986qv}
  L.~J.~Dixon, D.~Friedan, E.~J.~Martinec and S.~H.~Shenker,
 ``The Conformal Field Theory Of Orbifolds,''
  Nucl.\ Phys.\  B {\bf 282}, 13 (1987).

\bibitem{Ibanez:1987pj}
  L.~E.~Ibanez, J.~Mas, H.~P.~Nilles and F.~Quevedo,
 ``Heterotic Strings In Symmetric And Asymmetric Orbifold Backgrounds,''
  Nucl.\ Phys.\  B {\bf 301}, 157 (1988).

\bibitem{Greene:1989ya}
  B.~R.~Greene, A.~D.~Shapere, C.~Vafa and S.~T.~Yau,
  ``Stringy Cosmic Strings And Noncompact Calabi-Yau Manifolds,''
  Nucl.\ Phys.\  B {\bf 337}, 1 (1990).

\bibitem{OrbsFull}
  J.~Davey, A.~Hanany and R.~K.~Seong,
 ``Counting Orbifolds,''
  JHEP {\bf 1006} (2010) 010
  [arXiv:1002.3609 [hep-th]].

\bibitem{OrbsIntro}
  J.~Davey, A.~Hanany, R.~-K.~Seong,
  ``An Introduction to Counting Orbifolds,''
    [arXiv:1102.0015 [hep-th]].

\bibitem{DouglasMoore96}
  M.~R.~Douglas and G.~W.~Moore,
 ``D-branes, Quivers, and ALE Instantons,''
  arXiv:hep-th/9603167.

\bibitem{DouglasMoore97}
  M.~R.~Douglas and B.~R.~Greene,
 ``Metrics on D-brane orbifolds,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 1}, 184 (1998)
  [arXiv:hep-th/9707214].
  
\bibitem{DouglasGreeneMorrison97}
  M.~R.~Douglas, B.~R.~Greene and D.~R.~Morrison,
 ``Orbifold resolution by D-branes,''
  Nucl.\ Phys.\  B {\bf 506}, 84 (1997)
  [arXiv:hep-th/9704151].

\bibitem{Muto:1997pq}
  T.~Muto,
  ``D-branes on orbifolds and topology change,''
  Nucl.\ Phys.\  B {\bf 521}, 183 (1998)
  [arXiv:hep-th/9711090].

\bibitem{Beasley:1999uz}
  C.~Beasley, B.~R.~Greene, C.~I.~Lazaroiu and M.~R.~Plesser,
  ``D3-branes on partial resolutions of abelian quotient singularities of
  Calabi-Yau threefolds,''
  Nucl.\ Phys.\  B {\bf 566}, 599 (2000)
  [arXiv:hep-th/9907186].

\bibitem{Klebanov:1998hh}
  I.~R.~Klebanov and E.~Witten,
 ``Superconformal field theory on threebranes at a Calabi-Yau  singularity,''
  Nucl.\ Phys.\  B {\bf 536}, 199 (1998)
  [arXiv:hep-th/9807080].
 
\bibitem{Acharya:1998db}
  B.~S.~Acharya, J.~M.~Figueroa-O'Farrill, C.~M.~Hull and B.~J.~Spence,
 ``Branes at conical singularities and holography,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 2}, 1249 (1999)
  [arXiv:hep-th/9808014].

\bibitem{BaggerLambert07}
  J.~Bagger and N.~Lambert,
 ``Modeling multiple M2's,''
  Phys.\ Rev.\  D {\bf 75}, 045020 (2007)
  [arXiv:hep-th/0611108].

\bibitem{BaggerLambert08a}
  J.~Bagger and N.~Lambert,
 ``Gauge Symmetry and Supersymmetry of Multiple M2-Branes,''
  Phys.\ Rev.\  D {\bf 77}, 065008 (2008)
  [arXiv:0711.0955 [hep-th]].

\bibitem{BaggerLambert08b}
  J.~Bagger and N.~Lambert,
 ``Comments On Multiple M2-branes,''
  JHEP {\bf 0802}, 105 (2008)
  [arXiv:0712.3738 [hep-th]].

  \bibitem{Gustavsson07}
  A.~Gustavsson,
  ``Algebraic structures on parallel M2-branes,''
  [arXiv:hep-th/0709.1260].

\bibitem{Gustavsson08}
  A.~Gustavsson,
 ``Algebraic structures on parallel M2-branes,''
  Nucl.\ Phys.\  B {\bf 811}, 66 (2009)
  [arXiv:0709.1260 [hep-th]].
  
\bibitem{ABJM08}
  O.~Aharony, O.~Bergman, D.~L.~Jafferis and J.~Maldacena,
 ``N=6 superconformal Chern-Simons-matter theories, M2-branes and their
 gravity duals,''
  JHEP {\bf 0810}, 091 (2008)
  [arXiv:0806.1218 [hep-th]].
  
\bibitem{Martelli:2008si}
  D.~Martelli and J.~Sparks,
 ``Moduli spaces of Chern-Simons quiver gauge theories and AdS(4)/CFT(3),''
  Phys.\ Rev.\  D {\bf 78}, 126005 (2008)
  [arXiv:0808.0912 [hep-th]].
  
\bibitem{Hanany:2008cd}
  A.~Hanany and A.~Zaffaroni,
 ``Tilings, Chern-Simons Theories and M2 Branes,''
  JHEP {\bf 0810}, 111 (2008)
  [arXiv:0808.1244 [hep-th]].

\bibitem{Hanany:2008gx}
  A.~Hanany and Y.~H.~He,
 ``M2-Branes and Quiver Chern-Simons: A Taxonomic Study,''
  arXiv:0811.4044 [hep-th].
     
\bibitem{Yamazaki:2008bt}
  M.~Yamazaki,
 ``Brane Tilings and Their Applications,''
  Fortsch.\ Phys.\  {\bf 56}, 555 (2008)
  [arXiv:0803.4474 [hep-th]].
  
\bibitem{Davey:2009bp}
  J.~Davey, A.~Hanany, J.~Pasukonis,
``On the Classification of Brane Tilings,''
  JHEP {\bf 1001 } (2010)  078.
  [arXiv:0909.2868 [hep-th]].
    
\bibitem{Kennaway:2007tq}
  K.~D.~Kennaway,
 ``Brane Tilings,''
  Int.\ J.\ Mod.\ Phys.\  A {\bf 22}, 2977 (2007)
  [arXiv:0706.1660 [hep-th]].
  
\bibitem{HananyOrlando10}
  A.~Hanany, D.~Orlando and S.~Reffert,
 ``Sublattice Counting and Orbifolds,''
  arXiv:1002.2981 [hep-th].

\bibitem{HananyZaff08}
  A.~Hanany, D.~Vegh and A.~Zaffaroni,
 ``Brane Tilings and M2 Branes,''
  JHEP {\bf 0903}, 012 (2009)
  [arXiv:0809.1440 [hep-th]].

\bibitem{Hanany:1997tb}
  A.~Hanany and A.~Zaffaroni,
 ``On the realization of chiral four-dimensional gauge theories using
  branes,''
  JHEP {\bf 9805}, 001 (1998)
  [arXiv:hep-th/9801134].
  
\bibitem{Hanany:1998ru}
  A.~Hanany, M.~J.~Strassler and A.~M.~Uranga,
 ``Finite theories and marginal operators on the brane,''
  JHEP {\bf 9806}, 011 (1998)
  [arXiv:hep-th/9803086].

\bibitem{HananyUranga98}
  A.~Hanany and A.~M.~Uranga,
 ``Brane boxes and branes on singularities,''
  JHEP {\bf 9805}, 013 (1998)
  [arXiv:hep-th/9805139].
   
\bibitem{Sloane97}
  M.~Bernstein, N.J.A.~Sloane and P.E.~Wright,
 ``On sublattices of the hexagonal lattice,''
  Discrete Math., 170(1-3):29-39 (1997).
  
\bibitem{RakNew}
  A.~Hanany and R.~K.~Seong,
 ``Symmetries of Abelian Orbifolds,''
  arXiv:1009.3017 [hep-th].

\bibitem{M2Crystal}
  S.~Lee, S.~Lee and J.~Park,
 ``Toric AdS(4)/CFT(3) duals and M-theory crystals,''
  JHEP {\bf 0705} (2007) 004
  [arXiv:hep-th/0702120].

\bibitem{Leung:1997tw}
  N.~C.~Leung and C.~Vafa,
  ``Branes and toric geometry,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 2} (1998) 91
  [arXiv:hep-th/9711013].

\bibitem{Morrison:1994fr}
  D.~R.~Morrison and M.~Ronen Plesser,
 ``Summing the instantons: Quantum cohomology and mirror symmetry in toric
 varieties,''
  Nucl.\ Phys.\  B {\bf 440} (1995) 279
  [arXiv:hep-th/9412236].

\bibitem{Imamura:2008fd}
  Y.~Imamura, K.~Kimura and M.~Yamazaki,
 ``Anomalies and O-plane charges in orientifolded brane tilings,''
  JHEP {\bf 0803} (2008) 058
  [arXiv:0801.3528 [hep-th]].

\bibitem{PeskinSc}
  Michael~E.~Peskin and Dan~V.~Schroeder
``An Introduction To Quantum Field Theory,''
Westview Press, 1995.

\bibitem{ClossetReview}
  C.~Closset,
  ``Toric geometry and local Calabi-Yau varieties: An introduction to toric
  geometry (for physicists),''
  arXiv:0901.3695 [hep-th].

\bibitem{Davey:2009qx}
  J.~Davey, A.~Hanany, N.~Mekareeya, G.~Torri,
  ``Higgsing M2-brane Theories,''
  JHEP {\bf 0911 } (2009)  028.
  [arXiv:0908.4033 [hep-th]].

\bibitem{Feng:2001xr}
  B.~Feng, A.~Hanany and Y.~H.~He,
  ``Phase structure of D-brane gauge theories and toric duality,''
  JHEP {\bf 0108}, 040 (2001)
  [arXiv:hep-th/0104259].

\bibitem{Feng:2002fv}
  B.~Feng, S.~Franco, A.~Hanany and Y.~H.~He,
  ``Unhiggsing the del Pezzo,''
  JHEP {\bf 0308}, 058 (2003)
  [arXiv:hep-th/0209228].

  \bibitem{Feng:2001bn}
  B.~Feng, A.~Hanany, Y.~H.~He and A.~M.~Uranga,
  ``Toric duality as Seiberg duality and brane diamonds,''
  JHEP {\bf 0112}, 035 (2001)
  [arXiv:hep-th/0109063].\\
   C.~E.~Beasley and M.~R.~Plesser,
  ``Toric duality is Seiberg duality,''
  JHEP {\bf 0112}, 001 (2001)
  [arXiv:hep-th/0109053].

\bibitem{Franco:2003ea}
  S.~Franco, A.~Hanany and Y.~H.~He,
  ``A trio of dualities: Walls, trees and cascades,''
  Fortsch.\ Phys.\  {\bf 52}, 540 (2004)
  [arXiv:hep-th/0312222].

\bibitem{Franco:2003ja}
  S.~Franco, A.~Hanany, Y.~H.~He and P.~Kazakopoulos,
  ``Duality walls, duality trees and fractional branes,''
  arXiv:hep-th/0306092.

\bibitem{Verlinde:2005jr}
  H.~Verlinde and M.~Wijnholt,
  ``Building the Standard Model on a D3-brane,''
  JHEP {\bf 0701} (2007) 106
  [arXiv:hep-th/0508089].

\bibitem{Malyshev:2007yb}
  D.~Malyshev,
  ``Del Pezzo singularities and SUSY breaking,''
  arXiv:0705.3281 [hep-th].

\bibitem{Conlon:2008wa}
  J.~P.~Conlon, A.~Maharana and F.~Quevedo,
  ``Towards Realistic String Vacua,''
  JHEP {\bf 0905} (2009) 109
  [arXiv:0810.5660 [hep-th]].

\bibitem{Blumenhagen:2008zz}
  R.~Blumenhagen, V.~Braun, T.~W.~Grimm and T.~Weigand,
  ``GUTs in Type IIB Orientifold Compactifications,''
  Nucl.\ Phys.\  B {\bf 815} (2009) 1
  [arXiv:0811.2936 [hep-th]].

\bibitem{Blumenhagen:2009gk}
  R.~Blumenhagen, J.~P.~Conlon, S.~Krippendorf, S.~Moster and F.~Quevedo,
  ``SUSY Breaking in Local String/F-Theory Models,''
  JHEP {\bf 0909} (2009) 007
  [arXiv:0906.3297 [hep-th]].

\bibitem{Blumenhagen:2009yv}
  R.~Blumenhagen, T.~W.~Grimm, B.~Jurke and T.~Weigand,
  ``Global F-theory GUTs,''
  arXiv:0908.1784 [hep-th].

\bibitem{Balasubramanian:2009tv}
  V.~Balasubramanian, P.~Berglund and I.~Garcia-Etxebarria,
  ``Toric Lego: A method for modular model building,''
  arXiv:0910.3616 [hep-th].

\bibitem{database}
\verb|http://malham.kent.ac.uk/grdb/index.php|  
  
\bibitem{toricfano4}
V.~V.~Batyrev,
 ``On the Classification of Toric Fano 4-folds'',
arXiv:math/9801107.

\bibitem{KMM1} 
J.~Kollar, Y.~Miyaoka, S.~Mori, 
``Rational connectedness and boundedness of Fano manifolds'', 
J. Differ. Geom. 36, No.3, 765-779 (1992).

\bibitem{KMM2} 
J.~Kollar, Y.~Miyaoka, S.~Mori, 
``Rational curves on Fano varieties'', 
in {\sl Classification of irregular varieties, minimal models 
and abelian varieties}, Proc. Conf., Trento/Italy 1990,
Lect. Notes Math. {\bf 1515}, 100-105 (1992).

\bibitem{isk1} 
V.~A.~Iskovskih,  
``Fano 3-folds I'',  
Math.  USSR-Izv,  485-527 (1977) 

\bibitem{isk2} 
V.~A.~Iskovskih,  
``Fano 3-folds II'', 
Math. USSR - Izv., 12, 469-506 (1978)

\bibitem{MM1} 
S.~Mori, S.~Mukai, 
``Classification  of  Fano  3-folds  with $B_2 >2$'', 
Manusripta Math. 36, 147-162 (1981)

\bibitem{MM2}  
S.~Mori, S.~Mukai, 
``On Fano 3-folds with  $B_2 > 2$'', in {\sl Algebraic varieties and analytic varieties},
Proc. Symp., Tokyo 1981, Adv. Stud. Pure Math. 1, 101-129 (1983)  

\bibitem{MM3} 
S.~Mori, S.~Mukai, 
``Classification of Fano $3$-folds with $B\sb 2\geq 2$. I'', 
in  {\sl  Algebraic and topological theories} 
Nagata, M. (ed.) et al.,  
Papers from the symposium dedicated to the
memory of Dr. Takehiko Miyata held in Kinosaki, 
October 30-November 9, 1984. Tokyo: Kinokuniya Company
Ltd. 496-545 (1986)

\bibitem{murre}
J.-P.~Murre, 
``Classification of Fano threefolds according to Fano and Iskovskih,''  in Algebraic threefolds, Proc. 2nd 1981 Sess. C.I.M.E., Varenna/Italy 1981,
Lect. Notes Math. 947, 35-92 (1982).

\bibitem{cutkosky}
S.~D.~Cutkosky, 
``On Fano 3-folds'', 
Manuscr. Math. 64, No.2, 189-204 (1989).

\bibitem{toricfano3}
V.~V.~Batyrev, 
``Toroidal Fano 3-folds'', 
Math. USSR-Izv. 19, 13-25 (1982)

\bibitem{Kreuzer:2007zy}
  M.~Kreuzer and B.~Nill,
  ``Classification of toric Fano 5-folds,''
  arXiv:math/0702890.

\bibitem{Oebro07b} 
  M.~{\O}bro, 
  ``An algorithm for the classification of smooth Fano polytopes,''
  arXiv:0704.0049.

\bibitem{Hanany:2009vx}
  A.~Hanany, Y.~-H.~He,
  ``Chern-Simons: Fano and Calabi-Yau,''
    [arXiv:0904.1847 [hep-th]].

\bibitem{Davey:Fano}
  J.~Davey, A.~Hanany, N.~Mekareeya, G.~Torri,
  ``M2-Branes and Fano 3-folds,''
    [arXiv:1103.0553 [hep-th]].

\bibitem{Forger:Molien}
   M.~Forger,
``Invariant Polynomials and Molien Functions,''
J. Math. Phys. 39 (1998) 1107-1141

  \bibitem{GAP4}
  The GAP~Group, \emph{GAP -- Groups, Algorithms, and Programming, 
  Version 4.4.10}; 
  2007,
  \verb+(http://www.gap-system.org)+.

\bibitem{VanRaamsdonk:2008ft}
  M.~Van Raamsdonk,
  ``Comments on the Bagger-Lambert theory and multiple M2-branes,''
  JHEP {\bf 0805}, 105 (2008)
  [arXiv:0803.3803 [hep-th]].

 \bibitem{Ueda:2008hx}
  K.~Ueda and M.~Yamazaki,
  ``Toric Calabi-Yau four-folds dual to Chern-Simons-matter theories,''
  arXiv:0808.3768 [hep-th].

\bibitem{Hanany:2008qc}
  A.~Hanany, N.~Mekareeya, A.~Zaffaroni,
 ``Partition Functions for Membrane Theories,''
  JHEP {\bf 0809 } (2008)  090.
  [arXiv:0806.4212 [hep-th]].

\bibitem{Imamura:2008qs}
  Y.~Imamura, K.~Kimura,
  ``Quiver Chern-Simons theories and crystals,''
  JHEP {\bf 0810 } (2008)  114.
  [arXiv:0808.4155 [hep-th]].

\bibitem{Park:1999ep}
  J.~Park, R.~Rabadan, A.~M.~Uranga,
  ``Orientifolding the conifold,''
  Nucl.\ Phys.\  {\bf B570 } (2000)  38-80.
  [hep-th/9907086].

\bibitem{Franco:2009sp}
  S.~Franco, I.~R.~Klebanov, D.~Rodriguez-Gomez,
  ``M2-branes on Orbifolds of the Cone over Q**1,1,1,''
  JHEP {\bf 0908 } (2009)  033.
  [arXiv:0903.3231 [hep-th]].

\bibitem{Davey:2009et}
  J.~Davey, A.~Hanany, N.~Mekareeya, G.~Torri,
  ``Brane Tilings, M2-branes and Chern-Simons Theories,''
    [arXiv:0910.4962 [hep-th]].

\bibitem{Petrini:2009ur}
  M.~Petrini, A.~Zaffaroni,
  ``N=2 solutions of massive type IIA and their Chern-Simons duals,''
  JHEP {\bf 0909 } (2009)  107.
  [arXiv:0904.4915 [hep-th]].

\bibitem{Fabbri:1999hw}
  D.~Fabbri, P.~Fre', L.~Gualtieri, C.~Reina, A.~Tomasiello, A.~Zaffaroni, A.~Zampa,
  ``3-D superconformal theories from Sasakian seven manifolds: New nontrivial evidences for AdS(4) / CFT(3),''
  Nucl.\ Phys.\  {\bf B577 } (2000)  547-608.
  [hep-th/9907219].

\bibitem{Forcella:2009bv}
  D.~Forcella,
 ``Master Space and Hilbert Series for N=1 Field Theories,''
   [arXiv:0902.2109 [hep-th]].

\bibitem{Greene:1996cy}
  B.~R.~Greene,
 ``String theory on Calabi-Yau manifolds,''
  arXiv:hep-th/9702155.

\bibitem{ClayMath2003}
 K.~Hori, S.~Katz, A.~Klemm, R.~Pandharipande, R.~Thomas, C.~Vafa, R.~Vakil, E.~Zaslow,
 ``Mirror Symmetry'', vol. 1 of Clay Mathematics Monographs, American Mathematical Society, 2003. 929 p.

\bibitem{Bouchard:2006ah}
  V.~Bouchard,
  ``Toric Geometry and String Theory,''
    [hep-th/0609123].

\bibitem{Franco:2006gc}
  S.~Franco and D.~Vegh,
  ``Moduli spaces of gauge theories from dimer models: Proof of the
  correspondence,''
  JHEP {\bf 0611} (2006) 054
  [arXiv:hep-th/0601063].

\bibitem{Dai:1989ua}
  J.~Dai, R.~G.~Leigh, J.~Polchinski,
  ``New Connections Between String Theories,''
  Mod.\ Phys.\ Lett.\  {\bf A4 } (1989)  2073-2083.

\bibitem{Kennaway2005}
  A.~Hanany and K.~D.~Kennaway,
  ``Dimer models and toric diagrams,''
  arXiv:hep-th/0503149.

\bibitem{Berenstein:2002ge}
  D.~Berenstein,
  ``Reverse geometric engineering of singularities,''
  JHEP {\bf 0204} (2002) 052
  [arXiv:hep-th/0201093].

\bibitem{Kim:2007ic}
  S.~Kim, S.~Lee, S.~Lee, J.~Park,
 ``Abelian Gauge Theory on M2-brane and Toric Duality,''
  Nucl.\ Phys.\  {\bf B797 } (2008)  340-370.
  [arXiv:0705.3540 [hep-th]].

\bibitem{Lambert:2008et}
  N.~Lambert, D.~Tong,
``Membranes on an Orbifold,''
  Phys.\ Rev.\ Lett.\  {\bf 101 } (2008)  041602.
  [arXiv:0804.1114 [hep-th]].

\bibitem{Fuji:2008yj}
  H.~Fuji, S.~Terashima, M.~Yamazaki,
``A New N=4 Membrane Action via Orbifold,''
 Nucl.\ Phys.\  {\bf B810 } (2009)  354-368.
  [arXiv:0805.1997 [hep-th]].

\bibitem{Benna:2008zy}
  M.~Benna, I.~Klebanov, T.~Klose, M.~Smedback,
  ``Superconformal Chern-Simons Theories and AdS(4)/CFT(3) Correspondence,''
  JHEP {\bf 0809 } (2008)  072.
  [arXiv:0806.1519 [hep-th]].

\bibitem{Imamura:2008nn}
  Y.~Imamura, K.~Kimura,
  ``On the moduli space of elliptic Maxwell-Chern-Simons theories,''
  Prog.\ Theor.\ Phys.\  {\bf 120 } (2008)  509-523.
  [arXiv:0806.3727 [hep-th]].

\bibitem{Hosomichi:2008jb}
  K.~Hosomichi, K.~-M.~Lee, S.~Lee, S.~Lee, J.~Park,
  ``N=5,6 Superconformal Chern-Simons Theories and M2-branes on Orbifolds,''
  JHEP {\bf 0809 } (2008)  002.
  [arXiv:0806.4977 [hep-th]].

\bibitem{Terashima:2008ba}
  S.~Terashima, F.~Yagi,
``Orbifolding the Membrane Action,''
  JHEP {\bf 0812 } (2008)  041.
  [arXiv:0807.0368 [hep-th]].

\bibitem{Kim:2008gn}
  N.~Kim,
``Bagger-Lambert theory on an orbifold and its relation to Chern-Simons-matter theories,''
  Phys.\ Rev.\  {\bf D81 } (2010)  086006.
  [arXiv:0807.1349 [hep-th]].

\bibitem{Imamura:2008dt}
  Y.~Imamura, K.~Kimura,
``N=4 Chern-Simons theories with auxiliary vector multiplets,''
  JHEP {\bf 0810 } (2008)  040.
  [arXiv:0807.2144 [hep-th]].

\bibitem{Aharony:2008gk}
  O.~Aharony, O.~Bergman, D.~L.~Jafferis,
``Fractional M2-branes,''
  JHEP {\bf 0811 } (2008)  043.
  [arXiv:0807.4924 [hep-th]].

\bibitem{Ooguri:2008dk}
  H.~Ooguri, C.~-S.~Park,
  ``Superconformal Chern-Simons Theories and the Squashed Seven Sphere,''
  JHEP {\bf 0811 } (2008)  082.
  [arXiv:0808.0500 [hep-th]].

\bibitem{Jafferis:2008qz}
  D.~L.~Jafferis, A.~Tomasiello,
  ``A Simple class of N=3 gauge/gravity duals,''
  JHEP {\bf 0810 } (2008)  101.
  [arXiv:0808.0864 [hep-th]].

\bibitem{Imamura:2008ji}
  Y.~Imamura and S.~Yokoyama,
``N=4 Chern-Simons theories and wrapped M-branes in their gravity duals,''
  Prog.\ Theor.\ Phys.\  {\bf 121} (2009) 915
  [arXiv:0812.1331 []].

\bibitem{Broomhead:2008an}
  N.~Broomhead,
 ``Dimer models and Calabi-Yau algebras,''
  arXiv:0901.4662 [].
 
\bibitem{Imamura:2009ur}
  Y.~Imamura,
  ``Monopole operators in N=4 Chern-Simons theories and wrapped M2-branes,''
  Prog.\ Theor.\ Phys.\  {\bf 121 } (2009)  1173-1187.
  [arXiv:0902.4173 [hep-th]].

\bibitem{Amariti:2009rb}
  A.~Amariti, D.~Forcella, L.~Girardello, A.~Mariotti,
``3D Seiberg-like Dualities and M2 Branes,''
  JHEP {\bf 1005 } (2010)  025.
  [arXiv:0903.3222 [hep-th]].

\bibitem{Kim:2009wb}
  S.~Kim,
 ``The Complete superconformal index for N=6 Chern-Simons theory,''
  Nucl.\ Phys.\  {\bf B821 } (2009)  241-284.
  [arXiv:0903.4172 [hep-th]].

\bibitem{Aganagic:2009zk}
  M.~Aganagic,
  ``A Stringy Origin of M2 Brane Chern-Simons Theories,''
  Nucl.\ Phys.\  {\bf B835 } (2010)  1-28.
  [arXiv:0905.3415 [hep-th]].

\bibitem{Klebanov:2009sg}
  I.~R.~Klebanov, G.~Torri,
  ``M2-branes and AdS/CFT,''
  Int.\ J.\ Mod.\ Phys.\  {\bf A25 } (2010)  332-350.
  [arXiv:0909.1580 [hep-th]].

\bibitem{Benishti:2009ky}
  N.~Benishti, Y.~-H.~He, J.~Sparks,
  ``(Un)Higgsing the M2-brane,''
  JHEP {\bf 1001 } (2010)  067.
  [arXiv:0909.4557 [hep-th]].

\bibitem{Taki:2009wf}
  M.~Taki,
  ``M2-branes Theories without 3+1 Dimensional Parents via Un-Higgsing,''
    [arXiv:0910.0370 [hep-th]].

\bibitem{Hanany:2001py}
  A.~Hanany, A.~Iqbal,
  ``Quiver theories from D6 branes via mirror symmetry,''
  JHEP {\bf 0204 } (2002)  009.
  [hep-th/0108137].

\bibitem{Franco:2002ae}
  S.~Franco, A.~Hanany,
  ``Geometric dualities in 4-D field theories and their 5-D interpretation,''
  JHEP {\bf 0304 } (2003)  043.
  [hep-th/0207006].

\bibitem{Feng:2004uq}
  B.~Feng, Y.~-H.~He, F.~Lam,
  ``On correspondences between toric singularities and (p,q) webs,''
  Nucl.\ Phys.\  {\bf B701 } (2004)  334-356.
  [hep-th/0403133].

\bibitem{Benvenuti:2004dw}
  S.~Benvenuti, A.~Hanany,
  ``New results on superconformal quivers,''
  JHEP {\bf 0604 } (2006)  032.
  [hep-th/0411262].

\bibitem{Lee:2006hw}
  S.~Lee,
  ``Superconformal field theories from crystal lattices,''
  Phys.\ Rev.\  {\bf D75 } (2007)  101901.
  [hep-th/0610204].

\bibitem{Hanany:2006uc}
  A.~Hanany, C.~Romelsberger,
  ``Counting BPS operators in the chiral ring of N=2 supersymmetric gauge theories or N=2 braine surgery,''
  Adv.\ Theor.\ Math.\ Phys.\  {\bf 11 } (2007)  1091-1112.
  [hep-th/0611346].

\bibitem{Lawrence:1998ja}
  A.~E.~Lawrence, N.~Nekrasov, C.~Vafa,
 ``On conformal field theories in four-dimensions,''
  Nucl.\ Phys.\  {\bf B533 } (1998)  199-209.
  [hep-th/9803015].

\bibitem{Hanany:1998sd}
  A.~Hanany, Y.~-H.~He,
``NonAbelian finite gauge theories,''
  JHEP {\bf 9902 } (1999)  013.
  [hep-th/9811183].

\bibitem{Luty:1995sd}
  M.~A.~Luty, W.~Taylor,
  ``Varieties of vacua in classical supersymmetric gauge theories,''
  Phys.\ Rev.\  {\bf D53 } (1996)  3399-3405.
  [hep-th/9506098].

\bibitem{Gaberdiel:1999ch}
  M.~R.~Gaberdiel, B.~Stefanski, Jr.,
  ``Dirichlet branes on orbifolds,''
  Nucl.\ Phys.\  {\bf B578 } (2000)  58-84.
  [hep-th/9910109].

